Generating Instructions at Different Levels of Abstraction

When generating technical instructions, it is often convenient to describe complex objects in the world at different levels of abstraction. A novice user might need an object explained piece by piece, while for an expert, talking about the complex object (e.g. a wall or railing) directly may be more succinct and efficient. We show how to generate building instructions at different levels of abstraction in Minecraft. We introduce the use of hierarchical planning to this end, a method from AI planning which can capture the structure of complex objects neatly. A crowdsourcing evaluation shows that the choice of abstraction level matters to users, and that an abstraction strategy which balances low-level and high-level object descriptions compares favorably to ones which don't.

==> construction-model.tex <==
\begin{figure}[t]
{\small
For notation, let the set $\HObjects$ contain what we call \emph{high-level objects} in the Minecraft environment:\\[-1.9em]
\begin{align*}
\HObjects = \{&\mathrm{bridge(x, y, z, length, width, orientation), floor(x, y, z, length, width, orientation),} \\&\mathrm{railing(x, y, z, length, orientation), row(x, y, z, length, orientation)} \\&\text{with } \mathrm{x, y, z, length, width \in \mathbb{N}, orientation \in \{north, south, east, west\}}\}
\end{align*}
The construction HTN domain is defined as follows:\\[-1.9em]
\begin{align*}
\cTaskNamesConstruction = \{&\abstractTaskName{build-}X \mid X \in \HObjects\}\\
\FSetConstruction = \{&\factName{block(x,y,z)} \mid x, y, z \in \mathbb{N}\}\\
\decmethodsConstruction = \{
  & \abstractTaskName{Build-railing}(x,y,z,len,east) \rightarrow \langle \taskName{put-block}(x,y,z), \taskName{put-block}(x+len-1,y,z), \\
  &\phantom{\abstractTaskName{Build-railing}(x,y,z,len,east) \rightarrow \langle}\abstractTaskName{build-row}(x+len-1,y,z,len,west) \rangle ,  \\
  &\abstractTaskName{Build-railing}(x,y,z,len,east)  \rightarrow \langle \taskName{put-block}(x,y,z), \abstractTaskName{build-row}(x,y,z,len, east), \\
  &\phantom{\abstractTaskName{Build-railing}(x,y,z,len,east)  \rightarrow \langle}\taskName{put-block}(x+len-1,y,z) \rangle , 
   \dots \}\\
   \tniConstruction = \phantom{\{}&\abstractTaskName{build-bridge}(0,0,0,3,5,north)
\end{align*}

The set of actions $\pTaskNamesConstruction$ includes the following actions with $x, y, z \in \mathbb{N}$:\\[-1.2em]
\begin{center}
\begin{tabular} {r|ccc}
  & \precond & \add & \del \\ \midrule
  \taskName{put-block(x,y,z)} & $\neg$ \factName{block(x,y,z)}\  & \{\factName{block(x,y,z)}\} & \{\}  %\\
\end{tabular}
\end{center}
}
  \caption{Summary of bridge construction
    model. \decmethodsConstruction only shows a subset of the methods
    available.\alvaro{We should decide if to remove length, width, and
      orientation from everywhere to simplify everything. It is not
      clear if we need it for anything and it makes our examples more
      verbose and complicated.}\joerg{well, as a reader, if these
      things were missing, I would immediately wonder how a bridge is
      supposed to be identified merely by a xyz
      position.}} \label{fig:sumbridgeconstruction}
\end{figure}

==> instruction-model.tex <==

\begin{figure}
{\small
\begin{align*}
   \FSetInstruction = \FSetConstruction \cup \{&\factName{knows-row}, \factName{knows-floor}, \factName{knows-railing}, \factName{knows-bridge}\} \\\cup\, \{&\factName{lastblock(x,y,z)} \mid x,y,z \in \mathbb{N} \}\\
   \cTaskNamesInstruction = \cTaskNamesConstruction \cup  \{&\abstractTaskName{ins-build-block}(x,y,z) \mid x,y,z \in \mathbb{N}\} \cup \{\abstractTaskName{ins-build-X} \mid X \in \HObjects\}\\
   \tniInstruction =~ &\abstractTaskName{ins-build-bridge}(0,0,0,3,5,north) %, 
   %\sinitInstruction = \emptyset \text{ all positions are empty, IF does not know any complex object}
\end{align*}
% 
The set of methods $\decmethodsInstruction$\joerg{not sure what this half-sentence is doing here}. The rows labeled \emph{L}, \emph{H}, and \emph{T} illustrate decompositions leading to different levels of abstraction:\\[-1.9em]
\begin{align*}
 \decmethodsInstruction = \{
   \abstractTaskName{ins-build-block}(x,y,z) \rightarrow &\langle \taskName{ins-block(x,y,z)}, \taskName{put-block(x,y,z)} \rangle, \\  
   [L]~ \abstractTaskName{Ins-build-railing}(x,y,z,len,east) \rightarrow &\langle\abstractTaskName{ins-build-block}(x,y,z), \abstractTaskName{ins-build-block}(x+len-1,y,z), \\&\phantom{\{}\abstractTaskName{ins-build-row}(x+len-1,y,z,len,west)\rangle,  \\
     [H]~ \abstractTaskName{Ins-build-railing}(x,y,z,len,east) \rightarrow &\langle\taskName{ins-railing}(x,y,z,len,east), \abstractTaskName{build-railing}(x,y,z,len,east)\rangle,  \\
  [T]~ \abstractTaskName{Ins-build-railing}(x,y,z,len,east) \rightarrow &\langle\taskName{ins-teach-start-railing}(x,y,z,len,east), \\&\phantom{\{}\abstractTaskName{ins-build-block}(x,y,z), \abstractTaskName{ins-build-block}(x+len-1,y,z), \\&\phantom{\{}\abstractTaskName{ins-build-row}(x+len-1,y,z,len,west), \\&\phantom{\{}\taskName{ins-teach-end-railing}(x,y,z,len,east)\rangle,  
\dots \}
\end{align*}

The set of actions $\pTaskNamesInstruction$ contains all actions from $\pTaskNamesConstruction$ as well as the following additional actions (with $X \in \HObjects$):\\
% 
\scalebox{0.98}{
\begin{tabular} {r|ccc}
  & \precond & \add & \del \\ \midrule
  \taskName{ins-block(x,y,z)} & \{\} & \{\factName{lastblock(x,y,z)}\} &  \{\factName{lastblock(x',y',z')} $\mid \forall $ \factName{x',y',z'}\}  \\
  \taskName{ins-X}  & \{\factName{knows-X}\} & \{\}  & \{\}\\
  \taskName{ins-teach-start-X}  & \{\}  & \{\}  & \{\} \\
  \taskName{ins-teach-end-X}  & \{\} & \{\factName{knows-X}\} & \{\} \\
\end{tabular}
}
}
\caption{Extension of the construction model to the instruction model.}
\label{fig:instruction_model}
\end{figure}


